Misleading Repurposing on Twitter

We present the first in-depth and large-scale study of misleading repurposing, in which a malicious user changes the identity of their social media account via, among other things, changes to the profile attributes in order to use the account for a new purpose while retaining their followers. We propose a definition for the behavior and a methodology that uses supervised learning on data mined from the Internet Archive's Twitter Stream Grab to flag repurposed accounts. We found over 100,000 accounts that may have been repurposed. We also characterize repurposed accounts and found that they are more likely to be repurposed after a period of inactivity and deleting old tweets. We also provide evidence that adversaries target accounts with high follower counts to repurpose, and some make them have high follower counts by participating in follow-back schemes. The results we present have implications for the security and integrity of social media platforms, for data science studies in how historical data is considered, and for society at large in how users can be deceived about the popularity of an opinion.

==> aaai22_withcopyright.tex <==
\def\year{2022}
%
%Filename: aaai22.sty
%
\typeout{Conference Style for AAAI for LaTeX 2e -- version for the AAAI-22 conference}
% WARNING: IF YOU ARE USING THIS STYLE SHEET FOR AN AAAI PUBLICATION, YOU
% MAY NOT MODIFY IT FOR ANY REASON. MODIFICATIONS (IN YOUR SOURCE
% OR IN THIS STYLE SHEET WILL RESULT IN REJECTION OF YOUR PAPER).
%
% WARNING: This style is NOT guaranteed to work. It is provided in the
% hope that it might make the preparation of papers easier, but this style
% file is provided "as is" without warranty of any kind, either express or
% implied, including but not limited to the implied warranties of
% merchantability, fitness for a particular purpose, or noninfringement.
% You use this style file at your own risk. Standard disclaimers apply.
% There are undoubtably bugs in this style. If you would like to submit
% bug fixes, improvements, etc. please let us know. Please use the contact form
% at www.aaai.org.
%
% Do not use this file unless you are an experienced LaTeX user.
%
%
% PHYSICAL PAGE LAYOUT
\setlength\topmargin{-0.25in} \setlength\oddsidemargin{-0.25in}
\setlength\textheight{9.0in} \setlength\textwidth{7.0in}
\setlength\columnsep{0.375in} \newlength\titlebox \setlength\titlebox{2.25in}
\setlength\headheight{0pt}  \setlength\headsep{0pt}
%\setlength\footheight{0pt}  \setlength\footskip{0pt}
\thispagestyle{empty} \pagestyle{empty}
\flushbottom \twocolumn \sloppy
% We're never going to need a table of contents, so just flush it to
% save space --- suggested by drstrip@sandia-2
\def\addcontentsline#1#2#3{}
% gf: PRINT COPYRIGHT NOTICE
\def\copyright@year{\number\year}
\def\copyright@text{Copyright \copyright\space \copyright@year,
Association for the Advancement of Artificial Intelligence (www.aaai.org).
All rights reserved.}
\def\copyright@on{T}
%\def\nocopyright{\gdef\copyright@on{}} % Copyright notice is required for AAAI-22 papers.
\def\copyrighttext#1{\gdef\copyright@on{T}\gdef\copyright@text{#1}}
\def\copyrightyear#1{\gdef\copyright@on{T}\gdef\copyright@year{#1}}
% gf: End changes for copyright notice (used in \maketitle, below)
% Title stuff, taken from deproc.
\def\maketitle{\par
\begingroup % to make the footnote style local to the title
\def\thefootnote{\fnsymbol{footnote}}
% gf: Don't see why we'd want the footnotemark to be 0pt wide
%\def\@makefnmark{\hbox to 0pt{$^{\@thefnmark}$\hss}}
\twocolumn[\@maketitle] \@thanks
\endgroup
% gf: Insert copyright slug unless turned off
\if T\copyright@on\insert\footins{\noindent\footnotesize\copyright@text}\fi
% gf: And now back to your regular programming
\setcounter{footnote}{0}
\let\maketitle\relax \let\@maketitle\relax
\gdef\@thanks{}\gdef\@author{}\gdef\@title{}\let\thanks\relax}
\long\gdef\affiliations #1{ \def \affiliations_{#1}}

\def\@maketitle{%
  \newcounter{eqfn}\setcounter{eqfn}{0}%
  \newsavebox{\titlearea}
  \sbox{\titlearea}{
    \let\footnote\relax\let\thanks\relax%
    \setcounter{footnote}{0}%
    \def\equalcontrib{%
      \ifnum\value{eqfn}=0%
        \footnote{These authors contributed equally.}%
        \setcounter{eqfn}{\value{footnote}}%
      \else%
        \footnotemark[\value{eqfn}]%
      \fi%
    }%
    \vbox{%
      \hsize\textwidth%
      \linewidth\hsize%
      \vskip 0.625in minus 0.125in%
      \centering%
      {\LARGE\bf \@title \par}%
      \vskip 0.1in plus 0.5fil minus 0.05in%
      {\Large{\textbf{\@author\ifhmode\\\fi}}}%
      \vskip .2em plus 0.25fil%
      {\normalsize \affiliations_\ifhmode\\\fi}%
      \vskip .5em plus 2fil%
    }%
  }%
%
  \newlength\actualheight%
  \settoheight{\actualheight}{\usebox{\titlearea}}%
  \ifdim\actualheight>\titlebox%
    \setlength{\titlebox}{\actualheight}%
  \fi%
%
  \vbox to \titlebox {%
    \let\footnote\thanks\relax%
    \setcounter{footnote}{0}%
    \def\equalcontrib{%
      \ifnum\value{eqfn}=0%
        \footnote{These authors contributed equally.}%
        \setcounter{eqfn}{\value{footnote}}%
      \else%
        \footnotemark[\value{eqfn}]%
      \fi%
    }%
    \hsize\textwidth%
    \linewidth\hsize%
    \vskip 0.625in minus 0.125in%
    \centering%
    {\LARGE\bf \@title \par}%
    \vskip 0.1in plus 0.5fil minus 0.05in%
    {\Large{\textbf{\@author\ifhmode\\\fi}}}%
    \vskip .2em plus 0.25fil%
    {\normalsize \affiliations_\ifhmode\\\fi}%
    %{%
    %  \begin{tabular}[t]{p{\textwidth}}%
    %    \centering \Large{\textbf \@author}\ifhmode\\\fi%
    %    \vspace{3pt}  \normalsize  \affiliations_\ifhmode\\\fi%
    %  \end{tabular}%
    %}%
    \vskip .5em plus 2fil%
  }%
}%
%
\renewenvironment{abstract}{%
  \centerline{\bf Abstract}%
  \vspace{0.5ex}%
  \setlength{\leftmargini}{10pt}%
  \begin{quote}%
    \small%
}{%
  \par%
  \end{quote}%
  \vskip 1ex%
}%
% jsp added:
\def\pubnote#1{
  \thispagestyle{myheadings}%
  \pagestyle{myheadings}%
  \markboth{#1}{#1}%
  \setlength\headheight{10pt}%
  \setlength\headsep{10pt}%
}%
%
% SECTIONS with less space
\def\section{\@startsection {section}{1}{\z@}{-2.0ex plus
-0.5ex minus -.2ex}{3pt plus 2pt minus 1pt}{\Large\bf\centering}}
\def\subsection{\@startsection{subsection}{2}{\z@}{-2.0ex plus
-0.5ex minus -.2ex}{3pt plus 2pt minus 1pt}{\large\bf\raggedright}}
\def\subsubsection{\@startsection{subparagraph}{3}{\z@}{-6pt plus
%%% DIEGO changed: 29/11/2009
%% 2pt minus 1pt}{-1em}{\normalsize\bf}}
-2pt minus -1pt}{-1em}{\normalsize\bf}}
%%% END changed
\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}{-6pt plus -2pt minus -1pt}{-1em}{\normalsize\bf}}%
\setcounter{secnumdepth}{0}
% add period to section (but not subsection) numbers, reduce space after
%\renewcommand{\thesection}
%   {\arabic{section}.\hskip-0.6em}
%\renewcommand{\thesubsection}
%   {\arabic{section}.\arabic{subsection}\hskip-0.6em}
% FOOTNOTES
\footnotesep 6.65pt %
\skip\footins 9pt plus 4pt minus 2pt
\def\footnoterule{\kern-3pt \hrule width 5pc \kern 2.6pt }
\setcounter{footnote}{0}
% LISTS AND PARAGRAPHS
\parindent 10pt
\topsep 4pt plus 1pt minus 2pt
\partopsep 1pt plus 0.5pt minus 0.5pt
\itemsep 0.5pt plus 1pt minus 0.5pt
\parsep 2pt plus 1pt minus 0.5pt
\leftmargin 10pt \leftmargini 13pt \leftmarginii 10pt \leftmarginiii 5pt \leftmarginiv 5pt \leftmarginv 5pt \leftmarginvi 5pt
\labelwidth\leftmargini\advance\labelwidth-\labelsep \labelsep 5pt
\def\@listi{\leftmargin\leftmargini}
\def\@listii{\leftmargin\leftmarginii
\labelwidth\leftmarginii\advance\labelwidth-\labelsep
\topsep 2pt plus 1pt minus 0.5pt
\parsep 1pt plus 0.5pt minus 0.5pt
\itemsep \parsep}
\def\@listiii{\leftmargin\leftmarginiii
\labelwidth\leftmarginiii\advance\labelwidth-\labelsep
\topsep 1pt plus 0.5pt minus 0.5pt
\parsep \z@
\partopsep 0.5pt plus 0pt minus 0.5pt
\itemsep \topsep}
\def\@listiv{\leftmargin\leftmarginiv
\labelwidth\leftmarginiv\advance\labelwidth-\labelsep}
\def\@listv{\leftmargin\leftmarginv
\labelwidth\leftmarginv\advance\labelwidth-\labelsep}
\def\@listvi{\leftmargin\leftmarginvi
\labelwidth\leftmarginvi\advance\labelwidth-\labelsep}
\abovedisplayskip 7pt plus2pt minus5pt%
\belowdisplayskip \abovedisplayskip
\abovedisplayshortskip 0pt plus3pt%
\belowdisplayshortskip 4pt plus3pt minus3pt%
% Less leading in most fonts (due to the narrow columns)
% The choices were between 1-pt and 1.5-pt leading
\def\normalsize{\@setfontsize\normalsize\@xpt{11}}   % 10 point on 11
\def\small{\@setfontsize\small\@ixpt{10}}    % 9 point on 10
\def\footnotesize{\@setfontsize\footnotesize\@ixpt{10}}  % 9 point on 10
\def\scriptsize{\@setfontsize\scriptsize\@viipt{10}}  % 7 point on 8
\def\tiny{\@setfontsize\tiny\@vipt{7}}    % 6 point on 7
\def\large{\@setfontsize\large\@xipt{12}}    % 11 point on 12
\def\Large{\@setfontsize\Large\@xiipt{14}}    % 12 point on 14
\def\LARGE{\@setfontsize\LARGE\@xivpt{16}}    % 14 point on 16
\def\huge{\@setfontsize\huge\@xviipt{20}}    % 17 point on 20
\def\Huge{\@setfontsize\Huge\@xxpt{23}}    % 20 point on 23

\AtBeginDocument{\@ifpackageloaded{natbib}
  {
    % When natbib is in use, set the proper style and fix a few things
    \let\cite\citep
    \let\shortcite\citeyearpar
    \setcitestyle{aysep={}}
    \setlength\bibhang{0pt}
    \bibliographystyle{aaai22}
  }{}
}

\let\endthebibliography=\endlist

